Learning Under Moral Hazard with Instrumental Regression and Generalized Method of Moments

Machine learning has become increasingly popular in informing data-driven policy-making. Policies influence behavior in individuals or populations, and ideally, through observational signals, policy-makers learn which policies are effective. However, in many settings, individual actions cannot be perfectly observed. This issue, known in economics as moral hazard, poses a significant challenge. In this work, we study the foundational multitasking principal-agent contract design problem and demonstrate how instrumental regression and the generalized method of moments (GMM) estimator can be used to estimate or learn a good contract. As a bonus result, we also give a uniformity characterization of the shape of the optimal contract.

==> AISTATS2026PaperPack/AISTATS_checklist.tex <==

\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
The checklist follows the references. For each question, choose your answer from the three possible options: Yes, No, Not Applicable.  You are encouraged to include a justification to your answer, either by referencing the appropriate section of your paper or providing a brief inline description (1-2 sentences). 
Please do not modify the questions.  Note that the Checklist section does not count towards the page limit. Not including the checklist in the first submission won't result in desk rejection, although in such case we will ask you to upload it during the author response period and include it in camera ready (if accepted).

\textbf{In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.}
% %%% END INSTRUCTIONS %%%


\begin{enumerate}

  \item For all models and algorithms presented, check if you include:
  \begin{enumerate}
    \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
    \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
    \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Yes]
  \end{enumerate}

  \item For any theoretical claim, check if you include:
  \begin{enumerate}
    \item Statements of the full set of assumptions of all theoretical results. [Yes]
    \item Complete proofs of all theoretical results. [Yes]
    \item Clear explanations of any assumptions. [Yes]     
  \end{enumerate}

  \item For all figures and tables that present empirical results, check if you include:
  \begin{enumerate}
    \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes]
    \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Not Applicable]
    \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
    \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not Applicable]
  \end{enumerate}

  \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
  \begin{enumerate}
    \item Citations of the creator If your work uses existing assets. [Not Applicable]
    \item The license information of the assets, if applicable. [Not Applicable]
    \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
    \item Information about consent from data providers/curators. [Not Applicable]
    \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
  \end{enumerate}

  \item If you used crowdsourcing or conducted research with human subjects, check if you include:
  \begin{enumerate}
    \item The full text of instructions given to participants and screenshots. [Not Applicable]
    \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
    \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
  \end{enumerate}

\end{enumerate}


==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}



\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper's main contribution and scope are summarized inthe abstract and introduction. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper has section discussing the limitations. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All assumptions are clearly stated, and each for each theoretical result a complete proof is included. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Though this paper does not have large scale experiments, there are some numerical simulations that validate theoretical results. For the numerical simulations, enough details are provided for reproducibility. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: I currently did not release code. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Details are provided for the numerical experiments. 
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: I don't think this applies to the experiments in this paper. In particular, there is not a notion of ``mean" in the experiments. The experiments serve to show a quantity (the cumulative loss in an online learning problem) aligns with the upper bound in theoretical results. However, I did repeat the experiments multiple times. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The numerical experiments are ran on a personal laptop, which I also mentioned in the paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The reesearch conform to the Code of Ethics. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: I discussed positive impacts and do not foresee negative impacts. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This item does not apply. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This item does not apply. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This item does not apply. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This item does not apply. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This item does not apply. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> old/diversity-old.tex <==

\section{Diversity}
We now show when there is sufficient diversity in the agents, the regret bound can be significantly improved. We consider a special case where each agent's type is represented by a $d$-dimensional vector $k$, and that the cost function of this agent is
\[
c(w) = \frac{1}{2}  w' \diag(k)^{-1} w
\]
This implies that the agent's response when facing contract $\beta$ will be $\diag(k)\beta$. 

The goal here is then to show when $K_{\set{t}}$ is diverse, e.g., $K_t$ is sampled from some distribution and it satisfies some min eigenvalue condition, then one can actually achieve a $O(d\log T)$ regret with the naive GMM estimator. 

\begin{assumption}
The agent's type $k$ is sampled from some distribution $D$ at each round. Moreover, $\lambda_{\min} \Ex[k k^\top] \ge \lambda_0$. 
\end{assumption}

\begin{algorithm}
\caption{An Exploration-Free Algorithm}
\begin{algorithmic}
\For {$t = 1,\dots, d$}
    \State Query $\beta = (1, 0)$
\EndFor
\State Use Epoch based schedule
\For {$t = d+1,\dots, T$} 
    \State Compute $\theta_t = (Z'_t X_t)^{-1} Z'_t Y_t$
    \State Set $\beta_t = \theta_t / k$ \quad ($k = 2$ when agent's have quadratic costs)
\EndFor
\end{algorithmic}
\end{algorithm}

Another equivalent way to write $\theta$:
\[
err = (X^\top P_Z X)^{-1} X^\top P_Z y
\]
where
\[
P_Z = Z  (Z^\top Z)^{-1} Z^\top
\]

Idea 1:
First show $X^\top P_Z y$ is on the order of $\sqrt{T}$. Then some how upper bound the maximum eigenvalue of $(X^\top P_Z X)^{-1}$, or equivalently lower bound the minimum eigenvalue of $(X^\top P_Z X)$. But here $P_Z$ has a very small eigenvalue, however, would it be possible that the eigenvalue >= O(1)? 

Idea 2: In each epoch, where the epoch has length $t$, we add a small perturbation $u_t$, where
\[
\beta_t = \hat{\beta} + u_t, \norm{u_t} = 1/\sqrt{t}. 
\]
At the end of the epoch, the error term is
\[
(Z'X)^{-1} Z'\eta. 
\]
The term (recall $Z$ is a $t\times d$ matrix)
\begin{align*}
Z'\eta &= \sum z_i \eta_i \\
&= \sum (z + u_i) \eta_i \\
&= z t \eta_i + \sum_t u_i \eta_i \\
&= z O(\sqrt{t}) + O(1) ?
\end{align*}

We first bound the quantity
\[
(Z'X)^{-1} z \cdot O(\sqrt{t}) =? 1/\sqrt{t}
\]
\begin{align*}
z' (X' Z)^{-1} (Z' X)^{-1} z &= z' (Z' X X' Z)^{-1} z \\
&= 
\end{align*}

\begin{align*}
\sum_t u_i \eta_i = O(1)
\end{align*}

We need to bound the singular value of $Z' X$. 
\begin{align*}
\sigma_{\min} = \min_v \norm{X' Z v} \ge 1 / \sqrt{t} 
\end{align*}

\begin{lemma}
At the end of epoch $e$, we have $\norm{\theta_e - \theta}_2^2 \le \frac{xx}{yy}$. 
\end{lemma}
\begin{proof}
fff
\end{proof}

\section{Diversity - new}
Suppose there are $d$ types of agents. The $i$-th type of agent is talented in task $i$, and his response to $\beta$ is $\diag(k^i) \beta$. Therefore, at each round, choose the instrumental variable as
\[
z = \diag(k^*) \beta. 
\]

It can be seen that $z$ is indeed a valid instrumental variable (?). Further, the expression 
\[
(Z'X)^{-1} Z e
\]
can be bounded by $1/\sqrt{t}$, for each round $t$. 

This is because the minimum eigenvalue of $Z'X$ can be lower bounded. 

Suppose that the principal can contract with each agent twice. Denote the observations by $x_1, x_2, y_1, y_2$. We will use $x_1$ as an IV for $y_2$. 

Note that the design matrix is then
\begin{align*}
x \hat{x'} &= (x + \eps) (x + \eps')' \\
&= x x' + \eps x + \eps \eps'
\end{align*}
The expected min eigenvalue after $T$ rounds is then $\Omega(T)$. The estimate is
\[
(X'X)^{-1} X'Y. 
\]
Norm is bounded by $\sqrt{1}/{t}$. 


==> old/learningMH.tex <==


\section{A 2S-UCB Algorithm}
The relationship between the variables can be described as follows. 
\[
\beta \rightarrow x \rightarrow y, x\rightarrow r. 
\]
Note that assuming the agent best responds, then
\[
x_i = k_i \beta_i, y_i = k_i \beta_i + \eps. 
\]
Thus at each round we can form a confidence region for the variable $k_i$ (first stage in instrumental variable regression). 

Using an optimistic of $k_i$, then we can estimate the parameter $\theta$ using LinUCB type approach. Note that in both stages, OFUL needs to be applied! This seems to make analysis particularly challenging. 

\begin{algorithm}
\begin{algorithmic}
\For {$t = 1, \dots, T$}
    \State Estimate $\tilde{K}_t = LCB(k_i)$. 
    \State Use $K_t$ to estimate $\theta$ and form a confidence ellipsoid. (Use $LCB(k_i)$? )
    \State Apply OFUL and select $\theta_t$:
    \[
    \theta_t = \arg\max_{\theta\in \cC_t(K_t)} \theta K \theta
    \]
    \State The above needs to be verified, actually we may need this
    \[
    \theta_t, K_t = \arg\max_{K, \theta\in \cC(K)} \theta^t K \theta
    \]
    \State Principal sets $\beta_t = \theta_t / 2$
    \State Principal observes $y_t$, $r_t$
    %\State If $\beta_i$ large, means we get more accurate estimate in $k_i$, and at same time more accurate estimate in direction of? 
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{lemma}
Bounding the regret. 
\end{lemma}
\proof
Let $\reg(t)$ denote the instantaneous regret at round $t$. Then
\begin{align*}
\reg(t) &= \frac{1}{4} \theta^\top K \theta - (\theta^\top{K\beta} - \beta^\top{K\beta}) \\
&= \frac{1}{4}\theta^\top K \theta - (\theta^\top{K\theta_t / 2} - \theta_t^\top{K\theta_t} / 4) \\
&\le O( \norm{\theta - \hat{\theta}}_2^2 )
\end{align*}
\endproof

\begin{lemma}
Denote $B_{t,i} = \sum_t \beta_{t,i}$. Then
\[
k^*_i - k_{t,i} <= \frac{1}{\sqrt{B_{t,i}}}
\]
\end{lemma}

\section{Bayesian Approach}
Assume a prior on $K$ and $\theta$. 

\iffalse
\section{Warmup: No noise}
Idea 1. When there is no noise, the problem is simpler. Each round post $\beta$, observe $a$ and reward. A confidence ellipsoid can be computed from $(a,r)$ pair. But given this confidence ellipsoid, how should the learner choose the next action? 

Idea 2: thompson sampling. Maintain a distribution over $\Theta$. After observe $(a,r)$, update the posterior. Then each round, sample $\theta$ from the distribution and play $\theta / k$. 

Idea 3: Instrument variable regression

Idea 4: slightly perturb the contract to guarantee diversity condition met, though this would led to linear regret if not careful

\section{Learning the optimal linear contract}
The causal relationship can be specified as follows. 
\begin{align*}
\beta \rightarrow a \rightarrow y \\
a\rightarrow r
\end{align*}

We use ideas from Thompson sampling and the method of instrumental variables. Assume the cost is parameterized by $\psi$, in other words, $c(a) = c(a; \psi)$ Assume there is a prior 
\[
\Pr[ \psi, \theta ]
\]
We want to compute the posterior
\[
\Pr[\psi, \theta | y, r] \propto \Pr[y , r | \psi, \theta] \Pr[\psi, \theta]
\]

Note that the likelihood functions are well-defined
\begin{align*}
&\Pr[ y | \psi, \theta ] = \Pr[ y | \psi ] \\
&\Pr[ r | \psi, \theta ] 
\end{align*}
Therefore the likelihood can be computed as
\[
\Pr[ y, r | \psi,\theta ] = \Pr[r | \psi, \theta ] \Pr[y | \psi]
\]

% At each round, the principal posts a contract $\beta$, the agent responds with $a$, the signal $y$ is generated. They satisfy
% \[
% y = a - \eps. 
% \]
% The reward is
% \[
% r_t = \ip{\theta}{a} + \eps
% \]
% Note
% \[
% r_t = \ip{\theta}{y} + \ip{\theta}{\eps}. 
% \]
% We can no longer apply naive linear bandit algorithms since $y$ and $\eps$ are correlated. 

% In standard linear bandit,
% \[
% \Ex[r_t|y] = \ip{\theta}{y}
% \]
% But in ours
% \[
% \Pr[y | a] = N(a, I)
% \]
\fi





==> old/problemDescription.tex <==
\section{An unknown $\theta$}
We consider the setting where $\theta$ is unknown and must be learnt. We make the observation that this can be cast as an instrumental variable regression problem. Specifically, the causal relationship can be summarized as follows:
\begin{align*}
    \text{contract } \beta \rightarrow & \text{ action } x\rightarrow \text{signal } y\\
    &\text{action } x \rightarrow \text{outcome } r = \ip{\theta}{x} + \text{noise}
\end{align*}
Here, the contract $\beta$ acts as the IV, the signal $y$ is the dependent variable measured with error, and $\theta$ is the parameter of interest. 

By the uniformity result, the optimal contract only depends on $\theta$. In order to estimate $\theta$, we use the generalized method of moments (GMM) approach. 

\begin{algorithm}
\begin{algorithmic}
\State Estimate 
\end{algorithmic}
\end{algorithm}

% \section{Problem Description}
% Consider the multitasking principal-agent problem. The principal is risk-neutral and the agent is risk-averse with CARA utility function. There are $d$ tasks. The principal offers a contract $(\beta, w) \in \bbR^{d}\times \bbR$. When the agent takes action $a$, his certainty equivalent is:
% \[
% \dots. 
% \]

% The interaction protocol can be summarized as follows:
% \begin{enumerate}
% %\item The principal observes the context $M_t$
% \item The principal posts a contract $(\beta, w)$
% \item The agent responds with action $x$; however $x$ is unobserved
% \item The principal observes $y$, which is a noisy signal that depends on $x$
% \item The principal observes the outcome $r_t = \ip{\theta}{x} + \text{noise}$, and enjoys utility $r_t - \ip{\beta}{y} - w$
% \end{enumerate}
% Assume the agent has a quadratic cost function:
% \[
% c(x) = \frac{1}{2} xK^{-1}x = \sum \frac{1}{2k_i} x_i^2. 
% \]
% Then under the contract $(\beta,w)$, the incentive compatible action is
% \[
% x_i = k_i \beta_i. 
% \]
% The principal's optimal contract is then captured by the below program:
% \begin{align*}
% & \max_{\beta, w} \ip{\theta}{K \beta} - \ip{\beta}{K\beta} - w \\
% \text{s.t. } & \frac{1}{2} \ip{\beta}{K\beta} + w - \frac{r}{2}\norm{\beta}_2^2 \ge U_0. 
% \end{align*}

% Or
% \[
% \max_{\beta} \ip{\theta}{K\beta} - 0.5\ip{\beta}{K\beta} - (U_0 + \frac{r   }{2}\norm{\beta}_2^2)
% \]

% \paragraph{Parameters: which are known} In this program, $\theta$, the dependence of the agent's action on the outcome; $K$, the parameter describing the agent's cost function; and $U_0$, the parameter describing the agent's outside option, are unknown. We assume $r$, the parameter describing the agent's risk-averseness, is known. 

% \paragraph{What can be observed} At each round, the principal chooses the contract $(\beta, w)$, which is known to both parties once chosen. The agent can decide whether or not to participate in the contract, and this binary decision is observed. If the agent decides to enter the contract, the agent responds with $x$, and a signal $y$ is generated. $x$ is unobserved and $y$ is observed. The outcome cannot be exactly observed, instead the principal observes a noisy outcome:
% \[
% r_t = \ip{\theta}{x} + \text{noise}. 
% \]

% \paragraph{The optimal contract}
% The optimal contract is specified as follows:
% \[
% \beta_i = \frac{\theta_i}{1 + r \sigma^2 / k_i}. 
% \]
% And $w$ is the wage that binds the participation constraint. 



%The agent takes action $a$ such that $\beta = \nabla c(a)$. We assume the cost of the agent takes the quadratic form:
% \[
% c(x) = \sum \frac{1}{2 k_i} x_i^2. 
% \]
% So that when the posted contract is $\beta$, the best response of the agent is
% \[
% x_i = k_i \beta_i. 
% \]


% However, the action of the agent cannot be exactly observed, and only a noisy signal $y$ is generated. We assume
% \[
% \Ex[y | x] = x. 
% \]

% The outcome is given by
% \[
% r_t = \theta^\top x + \text{noise}. 
% \]




% \section{Problem Description}
% \subsection{No Moral Hazard}
% We consider the following optimization problem
% \[
% \ip{\theta}{x} - c(x)
% \]
% Here $c$ is a strictly convex function and is known. $\theta$ is the unknown parameter. 


% \subsection{Moral Hazard}
% The problem setup is as follows. The principal wishes to produce a certain product. She hires an agent to do so. The value of the product is determined by its intrinsic quality $x$. However, it will be costly for the agent to improve the quality of the product. Specifically, to achieve an intrinsic quality $x$, the agent must exert effort $\frac{1}{k} x^2 / 2$. We will refer to the value for the product as the outcome. The outcome each period is given by the equation:
% \[
% z = \theta \cdot x + \eps, \text{$\eps$ is noise term, independent of anything else}
% \]
% Moreover, the intrinsic quality cannot be directly observed, only a noisy signal $y$ can be observed. They satisfy the following
% \[
% y = x + \eps', \text{$\eps$ is noise term, independent of anything else}
% \]
% The principal must incentive the agent to improve the quality via a contract $\beta$, under which the agent is promised a payment $\beta y$. 

% The interaction protocol in each period is then summarized as follows:
% \begin{enumerate}
%     \item Principal posts contract $\beta$. 
%     \item Agent best responds with $x$, unobserved to the principal
%     \item Signal $y$ is generated, observed by both parties
%     \item Principal pays $\beta\cdot y$ to the agent, her utility is $z - \beta \cdot y$. 
% \end{enumerate}

% \section{Problem Description: Multitasking}
% The multitasking principal-agent problem can be specified as follows. The principal delegates $n$ tasks for an agent to perform. The agent can choose to exert an effort vector $x\in \bbR^n$. The effort is unobservable, but a noisy signal $y$ will be generated. The signal $y$ will only 
% (stochastically) depend on the effort profile $a$. Specifically, we make the assumption that
% \[
% y = x + \eps, \quad \text{$\eps$ is noise term with 0 mean, think gaussian for now}
% \]
% The reward to the principal is a linear function of the true effort $a$:
% \[
% r = \ip{\theta}{x}. 
% \]
% Here, $\theta$ is a vector unknown to the principal. 

% Exerting effort is costly for the agent. The cost function is given by $c(\cdot)$. We assume that $c$ takes the diagonal quadratic form
% \[
% c(x) = \frac{1}{2}x K^{-1} x, \quad \text{$K$ is diagonal matrix, it will be clear why we are using the inverse later}
% \]
% The principal must incentivize the agent to exert effort through contracts. A contract $\beta\in \bbR^n$ promises a payment
% \[
% \ip{\beta}{y}
% \]
% to the agent. 

% Therefore, the net utility of the principal is
% \[
% \text{reward $-$ payment} = \ip{\theta}{x} - \ip{\beta}{y}. 
% \]
% The interaction protocol in each period can now be specified as follows:
% \begin{enumerate}
% \item The principal posts a contract $\beta$
% \item The agent best responds with unobservable action $x$
% \item A signal $y = x + \eps$ is generated and observed by both parties
% \item The principal observes the reward $\ip{\theta}{x}$, then pays $\ip{\beta}{y}$ to the agent. 
% \end{enumerate}
% \begin{lemma}
% The optimal contract is $\beta = \theta / 2$, regardless of the shape of $K$. 
% \end{lemma}

==> old/uniform.tex <==
\section{A uniformity result in the multitasking problem}
The starting point of this work is the multitasking principal-agent problem. This problem was initially introduced in Holmstrom and Milgrom. In the multitasking problem, the principal hires an agent to complete $d$ tasks. In this work we assume both parties are risk-neutral. The agent takes a private action $x$ and incurs a cost $c(x)$. The action cannot be exactly observed, and a noisy signal $y$ is generated. We assume 
\[
y = x + \text{gaussian}. 
\]

The principal posts a contract $\beta \in \bbR^{d}$. The payment when signal $y$ is observed, is $\ip{\beta}{y}$. The agent should perform the following to find his best response
\[
x = \arg\max_{x'} \ip{\beta}{x'} - c(x'),
\]
Since the right-hand side is exactly his expected utility when taking action $x'$. Assuming interior solution, the first-order condition is satisfied:
\[
\beta = \nabla c(x). 
\]

Assuming when the agent takes action $x$, a private benefit $\ip{\theta}{x} + \text{noise}$ is enjoyed by the principal. 

\begin{theorem}
Assume the cost $c$ is homogeneous with degree $k$. The contract $\beta = \theta / k$ maximizes principal's utility. 
\end{theorem}
\begin{proof}
The principal's expected utility, as a function of $x$, is
\[
\ip{\theta}{x} - \ip{\beta}{x} = \ip{\theta}{x} - \ip{\nabla c(x)}{x} = \ip{\theta}{x} - kc(x)
\]
Taking the first order condition again,
\[
\theta = k\nabla c(x). 
\]
Also $\beta = \nabla c(x)$ (by agent's foc), therefore $\beta = \theta / k$ is the optimizer. 
\end{proof}

==> old/uniformity.tex <==
\section{Uniformity of the Optimal Linear Contract}
\subsection{Problem Statement}
The principal and agent are risk-neutral. The action set available to the learner is $A = (\bbR^+)^n$. When the agent takes action $a \in A$, his cost is $c(a) \in \bbR^+$, and the expected outcome (e.g. units of goods) is $f(a) \in \bbR^+$. The utility to the risk-neutral principal will then be exactly $f(a)$. The principal offers a linear contract parameterized by $\beta \in [0,1]$. Under this contract, the agent takes the action $a$ maximizing his expected utility:
\[
a(\beta) = \max_{a\in A} \beta f(a) - c(a). 
\]
The principal finds the best contract $\beta$ maximizing her utility:
\begin{align*}
\max_{\beta} & (1 - \beta) f(a) \\
\text{s.t. } & a = a(\beta). 
\end{align*}

Consider the function $\rho(a) = (\frac{\partial c(a) / \partial a_1}{\partial f(a) / \partial a_1}, \dots, \frac{\partial c(a) / \partial a_n}{\partial f(a) / \partial a_n})$. I impose the Inada conditions on the function $\rho(a)$. 
\begin{condition}
$\rho(a)$ is continuous and strictly increasing in each coordinate. Moreover,
\[
\frac{\partial c(a) / \partial a_i}{\partial f(a) / \partial a_i} |_{a_i \rightarrow 0^+} = 0, 
\]
\[
\frac{\partial c(a) / \partial a_i}{\partial f(a) / \partial a_i} |_{a_i \rightarrow +\infty} = +\infty. 
\]
\end{condition}

\subsection{The First Uniformity Result}

\begin{assumption}
$f$ is concave and homogeneous with degree $k_1 \le 1$. $c$ is convex and homogeneous with degree $k_2 > 1$. 
\end{assumption}

\begin{theorem}
Under the above assumption, the optimal linear contract is $\beta = \frac{k_1}{k_2}$. 
\end{theorem}
\begin{proof}
Given contract $\beta$, the agent's problem is:
\[
\max_a \beta f(a) - c(a)
\]

This is a strictly concave function. The first-order condition is: 
\begin{align}\label{eq:agentFOC}
\beta \nabla f(a) = \nabla c(a) 
\end{align}


By Poincaré-Miranda's theorem (the generalization of the intermediate value theorem to higher dimensions) together with the generalized Inada conditions, there exists a unique $a$ such that the above equality holds. Further, by multiplying both sides by the vector $a$ and applying Euler's theorem, 
\[
\beta k_1 f(a) = k_2 c(a). 
\]
Hence, at the optimum of the agent's problem $a= a(\beta)$ we must have: 
\[
\beta = \frac{k_2 c(a)}{k_1 f(a)}. 
\]

When the posted contract is $\beta$, the principal's utility is:
\begin{align*}
(1 - \beta) f(a(\beta)) &= (1 - \frac{k_2 c(a)}{k_1 f(a)} ) f (a) \\
&= f(a) - \frac{k_2}{k_1} c(a)
\end{align*}

Note that this is a concave function with respect to $a$, although the domain is only restricted to those actions $a$ that can be induced by linear contracts. However, if we can find some $a$ such that the first order condition (with respect to $a$) holds for the above concave problem, and that $a$ can be induced by some contract $\beta$, then this $a$ must be optimal for the principal's problem. 
Therefore, let us first examine the first-order condition:
\[
\nabla f(a) = \frac{k_2}{k_1}\nabla c(a). 
\]

Now, notice the first order condition is satisfied when $a$ is exactly the action induced by the contract $\beta = \frac{k_1}{k_2}$! \qedhere
% However, if we take $a$ to be the action induced by the contract $\beta = \frac{k_1}{k_2}$, the first order condition is indeed satisfied! 


% Nevertheless, there must exist some $a^*\in A$ that is the unique maximize to the above concave problem. At this point $a^*$, the first order condition must hold:
% \[
% \nabla f(a^*) = \frac{k_2}{k_1}\nabla c(a^*). 
% \]

% But this action $a^*$ can be exactly induced by the contract $\beta = \frac{k_1}{k_2}$! 

% If we set $\beta = \frac{k_1}{k_2}$, then by~\cref{eq:agentFOC}, the induced agent's action must satisfy:
% \[
% \frac{k_1}{k_2}\nabla f(a) = \nabla c(a)
% \]
% which in turn implies the principal's problem must be optimal! 
\end{proof}

\section{Uniformity of the Optimal Linear Contract in Multitasking}

\subsection{Problem Statement}

Let us now consider the multi-task principal-agent problem. The principal delegates $n$ tasks to the agent, and can observe an outcome for each task. I will assume the following: when the agent takes action $a \in (\bbR^+)^n$, the outcome is a random vector with mean $a$. The linear contract is a vector $\beta \in (\bbR^+)^n$, under which the expected payment to the agent is $\ip{\beta}{a}$. Given a contract $\beta$, the agent's maximization problem is
\[
\max_a \ip{\beta}{a} - c(a). 
\]
We assume the principal exhibits a linear utility function with marginals $u$, so that her optimization problem is:
\begin{align*}
\max_\beta &\ip{u}{a} - \ip{\beta}{a}, \\
\text{s.t. } &a = a(\beta)
\end{align*}

\subsection{The Second Uniformity Result}
\begin{assumption}
$c$ is homogenous with degree $k > 1$. 
\end{assumption}

\begin{theorem}
The optimal linear contract is $\beta = \frac{u}{k}$. 
\end{theorem}
\begin{proof}
Consider the agent's maximization problem. The first-order condition implies that the action $a$ satisfies:
\[
\beta = \nabla c(a). 
\]
The principal's utility is
\[
\max_\beta \ip{u}{a} - \ip{\beta}{a}. 
\]
Substituting $\beta = \nabla c(a)$ and applying Euler's theorem, the above becomes
\[
\ip{u}{a} - \ip{\nabla c(a)}{a} = \ip{u}{a} - k_2 c(a),
\]
which is a strictly concave function in $a$. Taking the derivative with respect to $a$:
\[
u = k_2 \nabla c(a). 
\]
Combined with the first-order condition on the agent's maximization problem $\beta = \nabla c(a)$, the optimal contract must satisfy: 
\[
\beta = \frac{u}{k_2}. 
\]
Hence, the optimal contract is then the contract that transfers a $1/k_2$ fraction of utility in each dimension. 
\end{proof}

\subsection{Optimality of Linear Contracts}
We next show without loss of generality we can assume the linear contract is linear. 

==> old/warmup.tex <==
\section{Warmup: No Moral Hazard}
The principal should optimize $\theta\cdot x - \frac{1}{2}x^2$. The optimal $x$ is $\theta$, but of course $\theta$ is unknown. 

At each round, the learner can construct a confidence bound for $\theta$ (as UCB), and should set $x_t$ as the UCB. This guarantees: 1. The learner is acting optismistically; 2. at each round, the learner is learning the maximum possible information. 

\begin{algorithm}
\begin{algorithmic}
\For {$t = 1,\dots,T$}
    \State Compute $\UCB(\theta) = \hat{\theta} + \frac{1}{\sqrt{X}}$
    \State Set $x = \UCB(\theta)$
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{lemma}
$\UCB(\theta) \in [\theta, \theta + \frac{1}{2\sqrt{X}}]$. 
\end{lemma}

\begin{theorem}
The regret can be bounded. 
\end{theorem}
\begin{proof}
The regret can be bounded:
\begin{align*}
\reg &= \frac{1}{2} \sum_{t} (x_t - \theta)^2 \\
&= \sum_t (\hat{\theta} + \frac{1}{\sqrt{X_t}} - \theta)^2 \\
&\le \sum_t \frac{1}{X_t} \\
&\le \sum_t \frac{1}{t \theta} \\
&\le \frac{\log T}{\theta}. 
\end{align*}
\end{proof}

\section{Instrumental Variable Regression}
Now consider when the cost function is unknown and given by $c(x) = x^2 / (2k)$, where $k$ is an unknown parameter. The causal relationship can be specified by
\[
\beta \rightarrow x \rightarrow y, x \rightarrow z
\]
Of course, even though $\Ex[y|x] = x$ and $\Ex[z|x] = \theta\cdot x$, it would be a mistake to try to regress $z$ on $y$ and find the coefficient $\theta$. This corresponds to the error-in-measurement problem. However, we note $\beta$ acts as an instrumental variable. Therefore, we propose the following two-stage OFUL approach. 

\begin{algorithm}
\caption{2S-OFUL}
\begin{algorithmic}
\For {$t = 1,\dots,T$}
    \State Set $B_t := \sum_t \beta_t$
    \State Compute $\LCB(k), \UCB(k) = \hat{k} \pm \frac{1}{\sqrt{B_t}}$
    \State Set $X_t := \sum_t \LCB(k)\cdot \beta_t$
    \State Set $Z_t := \sum_t z_t$
    \State Compute $\UCB(\theta) = \frac{Z_t}{\LCB(X_t)} + \frac{1}{\sqrt{\LCB(X_t)}}$. 
    \State Compute $\LCB(\theta) = \frac{Z_t}{\UCB(X_t)} - \frac{1}{\sqrt{\UCB(X_t)}}$. 
    \State Then $\theta \in [\LCB(\theta), \UCB(\theta)]$. 
    \State Set $\beta_t = \UCB(\theta)$
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{lemma}
$\LCB(k) \in [k - 2\frac{1}{\sqrt{B_t}}, k]$
\end{lemma}

\begin{lemma}
$X_t$ can be bounded. 
\end{lemma}
\begin{proof}
$\LCB(X_t) = \LCB(k) \cdot B_t$, and $X_t = k \cdot B_t$. 
By the previous lemma
\[
\LCB(X_t) \in [k - 2\frac{1}{\sqrt{B_t}}, k] \cdot B_t = [X_t - 2\sqrt{B_t}, X_t]
\]
\end{proof}

\begin{lemma}
$\UCB(\theta) \in [\theta, \theta + \frac{\text{const}}{\sqrt{\LCB(X_t)}}]$. 
\end{lemma}

\begin{theorem}
The regret can be bounded. 
\end{theorem}
\proof
\begin{align*}
\reg &= \frac{1}{2} \sum_t (\beta_t - \theta)^2 \\
&\le \sum_t \frac{1}{\LCB(X_t)} \\
&\le \sum_t \frac{1}{X_t - 2\sqrt{B_t}} \\
&\le \frac{\log T}{\theta}? 
\end{align*}
\endproof

\subsection{Greedy?}
The estimation error probably converges at rate $1 / t$. 
\proof
\begin{align*}
\reg &= \sum (\beta_t - \theta)^2\\
&\le \sum_t \frac{1}{t}
\end{align*}
\proofname

\section{Results on Confidence Ellipsoid}
\subsection{Two stage: regress on $x$}
Define $V_t = X_T^\top X_T + \lambda I$. Define $\hat{\theta} = (X^\top X + \lambda I)^{-1}X_T^\top Y$. Here $X$ is the $t\times d$ matrix, where rows are the covariates of each time period. 

We are using estimates for $X$, which means $X = $
\begin{definition}
    The confidence ellipsoid is defined as
    \begin{align*}
    \set{\theta: \norm{\theta - \hat{\theta}}_{V_t} < \text{const}}
    \end{align*}
\end{definition}

\subsection{Regress on $\beta$}
Regress on $\beta$ seems like the better choice. Define $\phi = K\theta$. Then at each round, there is a confidence ellipsoid for $\phi$:
\[
\set{\phi: \norm{\phi - \hat{\phi}}_{B_t} \le \delta}
\]
And the confidence ellipsoid for $\theta$ can be estimated
\[
\cC(\theta) = K^{-1}\phi. 
\]
And from the confidence ellipsoid, the learner should somehow choose the best action... 

\section{Smoothed Analysis Approach}
The regret each round can be bounded by 
\begin{align*}
\norm{\theta^* - \beta_t}_2^2 \le \norm{\theta^* - \hat{\theta}}_2^2 + \norm{\hat{\theta} - \beta_t}_2^2
\end{align*}
\begin{lemma}
$\norm{\hat{\theta} - \beta_t}_2^2 \le \frac{\text{const}}{\lambda_{\min}(B_t)}$. 
\end{lemma}
\begin{proof}
??
\end{proof}

\begin{lemma}
$\norm{\theta^* - \hat{\theta}}_2^2 \le ???$. 
\end{lemma}
\begin{proof}
$\hat{\theta} = \hat{K}^{-1} \hat{\phi} $. We know that
\[
\norm{\hat{\phi} - \phi}_{B_t} \le \text{const}
\]
And we need to bound
\[
\norm{ {K}^{-1} \phi - \hat{K}^{-1} \hat{\phi}} \le \frac{???}{\lambda_{\min}(B_t)}. 
\]
\end{proof}

Therefore, the key seems to be to lower bound $\lambda_{\min} (B_t)$. 

\subsection{Smoothed Analysis Approach}
Assuming smoothed analysis $\lambda_{\min}(B_t) \ge t$?. 

\section{The cost function is known}
Assume the cost function is $c(a) = \norm{a}_2^2$. Then each round, the response is exactly $x_t = \beta_t$. The regret each round is
\[
\norm{\theta^* - 2 x_t}_2^2
\]
Further an outcome $\ip{\theta}{\beta_t}$ is observed. 

\begin{algorithm}
\begin{algorithmic}
\For {$t = \dots, $}
    \State Construct confidence ellipsoid for $\theta$:
    \[
    \norm{\hat{\theta} - \theta}_{V_t} \le \delta
    \]
    \State Choose the $\theta_t$ maximizing $\norm{\theta_t}_2^2$. (Use this fact to show $\max_v v^\top V_t v$ is increasing. )
\EndFor
\end{algorithmic}
\end{algorithm}

Problem: Choose a $\theta_t$ in the confidence ellipsoid each round, so that the minimum eigenvalue of $V_t$ is minimized. Greedilty choose the $\theta_t$ that can minimize the new matrix $V_t$? 

\begin{theorem}
The total regret can be bounded. 
\end{theorem}
\proof
\begin{align*}
\sum \norm{\theta^* - \theta_t}_2^2 &= (\delta / \lambda_{\min}(V_t)) ^ 2
\end{align*}
And
\[
V_t = \sum \theta_t \theta_t^\top
\]
\endproof

Suppose the confidence ellipsoid were centered at $0$, then $\lambda_{\min}(V_t) \ge d/t$. Which suggests a $O(1)$ regret. 

\section{An Explore-Then-Commit Type algorithm}
The learner's problem is
\[
\max_\beta {\theta}K\beta - \beta K \beta
\]
a quadratic function in $\beta$. 

\begin{algorithm}
\begin{algorithmic}
\For{$t = 1, \dots, d \cdot T_0$}
    \State Post the contract $\beta = (0,0,\dots,1, 0,\dots, 0)$ for $T_0$ times. 
    \State Observe the average signal $\hat{y}_i$, average reward $\hat{r}_i$. 
\EndFor
\State Estimate the parameters $\hat{k}_i = \hat{y}_i$, set $\hat{x}_t = \hat{k}_i$
\State Estimate the parameter $\theta_i$ as 
\[
\hat{\theta}_i = \hat{r}_i / \hat{x}_i. 
\]
\State Set $\beta_i = \hat{\theta}_i / 2$ for the remaining rounds
\end{algorithmic}
\end{algorithm}

\begin{lemma}
After the explore phase, $\hat{k}_i - k_i < \frac{1}{\sqrt{T_0}}$. 
\end{lemma}
\begin{lemma}
$\theta_i - \hat{\theta}_i < \frac{1}{\sqrt{T_0}}$
\end{lemma}
\proof 
\begin{align*}
\hat{\theta}_i = \frac{\hat{r}_i}{\hat{x}_i} = \frac{{r}_i + \eps}{x_i + \eps'_i}
\end{align*}
\begin{align*}
\hat{\theta}_i - \theta_i &= \frac{{r}_i + \eps}{x_i + \eps'_i} - \frac{r_i}{x_i} \\
&\le \frac{\eps x_i - \eps'_i r_i}{(x_i + \eps'_i) x_i} \\
&\le T^{1/3}
\end{align*}
\endproof

\begin{theorem}
The regret can be bounded. 
\end{theorem}

\begin{proof}
The regret each period in the exploitation phase is
\begin{align*}
\reg(t) &= \sum_i k_i\theta_i^2 / 4 - (\sum_i k_i \theta_i \hat{\theta}_i / 2 - k_i \hat{\theta}_i^2 / 4) \\
&= \sum_i k_i (\theta_i - \hat{\theta}_i)^2 / 4 \\
&\le O(\norm{\theta - \hat{\theta}}_2^2) \\
&\le \frac{1}{T_0}
\end{align*}

Therefore total regret is $ T_0 + \frac{T}{T_0} = \sqrt{T}$. 
\end{proof}




==> sec/abstract.tex <==
In this work, we study the multitasking principal-agent problem. The agent performs several task for the principal, and the principal posts a contract incentivizing the agent to exert effort. The principal can observe a signal for each task, and the contract is a mapping from the space of possible signals to a payment. We study the special class of linear contracts from three perspectives: robustness, uniformity, and learning. Firstly, we show a robustness result: in an ambiguous setting when only first moment information is known, there is a linear contract maximizing the principal's payoff in a worst-case scenario. Secondly, we show a uniformity result: when the agent's cost function is homogeneous to a certain degree and the the principal's utility takes a linear form across tasks, then the optimal contract depends on the agent's cost function only through its homogeneuity degree. Thirdly, we study the problem of learning an optimal linear contract through observational data. We identify this as an measurement error model, and propose instrumental regression methods to estimate the optimal contract parameters in an offline setting, or to learn the optimal contract in an online setting. 


==> sec/conclusion_old.tex <==
\section{Conclusion}
In this work, we examined the role of linear contracts in principal-agent problems from three key perspectives: robustness, uniformity, and learning. 

Firstly, we analyzed the robustness properties of linear contracts. In an ambiguous principal-agent setting where only first-moment information is available, we demonstrated that a linear contract is worst-case optimal. This result underscores the resilience of linear contracts under uncertainty, providing a rationale for their widespread use in practical applications. A natural question for future research is to investigate the extent to which our assumptions can be relaxed while preserving the robustness guarantees. Understanding the boundary conditions of these results could yield deeper insights into the trade-offs between contract simplicity and performance in uncertain environments.


Second, we provided a theoretical justification for the use of uniform contracts when contracting with heterogeneous agents. Our analysis establishes conditions under which uniform contracts are not only feasible but also optimal. Specifically, when agents exhibit certain cost function properties, a uniform contract structure can align incentives effectively without the need for agent-specific tailoring. This result is particularly relevant in settings such as franchising or platform-based economies, where principals interact with diverse agents yet often employ standardized contracts.

Finally, we investigated the problem of learning optimal contracts in scenarios where the principal lacks complete knowledge of agent-specific parameters. We drew a connection between contract learning and instrumental regression, highlighting how techniques from causal inference can inform strategic contract design. Notably, recent research has recognized the relationship between learning in strategic settings and causal inference methods, such as instrumental regression. Building on this, a promising direction for future work is to explore how learning with strategic interactions in Stackelberg games can be framed within the instrumental regression framework. This could open new avenues for leveraging econometric techniques in the study of contract optimization.



% In this work we studied the use of linear contracts in principal-agent problems from three perspectives: uniformatiy, learning, and robustness. 

% We first gave a justification for the use of uniform contracts when contracting with hetergeneosu agents. [Chatgpt, say smth. ]

% We also studied the problem of learning the optimal contract and cast a link to the instrumental regression framework. We note that some recent work also note the relation between learning in strategic settings to causal inference methods such as instrumental regression. For future work, it may be interesting to see how one can cast learning with strategic interactions in Stackelberg games to instrumental regression methods. 

% Finally, we studied the robustness properties of linear contracts. We showed that in an ambiguous principal-agent problem where only first moment is available, a linear contract is worst-case optimal. Future work may examine to what extend the assumptions can be relaxed. 


% This work studied the multitask principal-agent problem. I first present a result justifying the use of uniform contracts when the principal contracts with heterogeneous agents. Then, I study the problem of learning the optimal contract and identify the problem as a measurement error problem, and propose using instrumental regression with the generalized method of moments estimator to estimate and learn the optimal contract. A limitation of the current work is that in the ``diversity'' condition in \Cref{sec:repeated}, the agents are limited to have quadratic cost functions. I believe this can be extended to more general cost functions (beyond quadratic functions and beyond $k = 2$). Specifically, the ``diversity'' condition will hold whenever there are some variations in the agent's ``abilities" in each task. I will leave a more formal treatment to future work. 


==> sec/introduction_old.tex <==
\section{Introduction}
A firm's owner (the principal) hires a manager (the agent) to perform multiple tasks, such as managing personnel, maintaining a healthy work environment, and executing strategic initiatives. The agent can allocate effort across these tasks, but this effort is unobservable and unverifiable to the principal. Instead, the principal receives noisy signals that indicate task performance and can observe the total revenue generated by the firm, which depends on the agent's effort allocation. To incentivize the agent, the principal offers a contract that links compensation to these noisy signals. Since direct effort observation is impossible, the contract structure plays a crucial role in aligning incentives. This setting defines the multitask principal-agent problem, first studied in the seminal work \cite{holmstrom1991multitask}.

A contract in a multitasking problem is a mapping from the signal space to a payment. In theory, such contracts can be highly complex. Even in the well-studied single-task setting, optimal contracts can exhibit significant complexity. However, empirical observations suggest that most contracts used in practice tend to be relatively simple. A particularly important class of simple contracts is linear contracts. Many recent works have examined linear contracts in single task settings from various perspectives, including robustness and approximation properties (e.g. \cite{dutting2019simple}, \cite{carroll2015robustness}). However, the role of linear contracts in multitask settings remains underexplored. In this work, we study linear contracts in multitask principal-agent problems from three key perspectives: robustness, uniformity, and learnability. 

\paragraph{Robustness. } Recent works have studied the robustness of linear contracts and established their optimality in ambiguous or non-Bayesian worst-case settings (e.g. \cite{carroll2015robustness}, \cite{dutting2019simple}). In this work, we extend these findings to the multitask principal-agent setting and provide a robustness guarantee under ambiguity. Our research question can be summarized as follows: 
\begin{center}
\emph{ Does the linear contract exhibit strong robustness guarantees in the multitask principal-agent setting? }
\end{center}
We show that when the principal knows only the first moment of each agent's action but lacks information about its full distribution, a linear contract remains optimal under the worst-case distribution. This result highlights the structural advantages of linear contracts in environments with uncertainty. Our findings are similar in spirit to the prior results in \cite{dutting2019simple}, which demonstrate the robustness of linear contracts in single-task settings. However, the transition to multitask environments introduces additional complexities, requiring new proof ideas; the crux of our proof contains a triangulation result from convex geometry followed by an application of Kakutani's fixed-point theorem. 



\paragraph{Uniformity.} In many real-world scenarios, the principal engages with multiple agents under the same contractual framework. A prominent example is franchising, where the principal (franchiser) contracts with multiple franchisees to ensure consistent effort and revenue generation \cite{bhattacharyya1995double}. Another example is e-commerce platforms such as YouTube, where content creators earn a share of advertising revenue. According to official documentation \cite{YouTubeShare}, YouTube content creators receive 55\% of the total advertisement revenue, while the remaining 45\% is retained by the platform. While one might expect the principal to tailor contracts for different agents to maximize utility, it is often observed that contracts remain uniform across agents. This observation leads to our second research question.

\begin{center}
\textit{How can the uniformity of contract terms be justified in multitask principal-agent problems?}
\end{center}

To answer this question, we show that when the agent’s cost function exhibits a certain degree of homogeneity and the principal’s utility is linear across tasks, the optimal contract is necessarily uniform across agents. Specifically, the optimal contract depends on the agent's cost function \emph{only through} it's the homogeneity degree. This result has strong practical implications: it suggests that the principal does not need to differentiate contracts to maximize utility, reinforcing fairness in contract design. Our findings are similar in spirit to the work of \cite{bhattacharyya1995double}, who examine a single-task setting with double moral hazard. In contrast, our study focuses on multitask environments. 

\paragraph{Learning} In the optimal contract, imaginably the principal should offer a higher incentives to tasks that are more ``important", i.e., tasks which have a higher marginal utility. However, the exact ``importance" of each task may not always be known. In such cases, the principal must infer these values from observational data to design the optimal contract. This naturally leads to our third research question:

\begin{center}
\textit{How can the principal learn the optimal contract when the ``importance'' of each task is unknown?}
\end{center}

Assuming that the principal’s utility remains linear across tasks, estimating the marginal utilities reduces to a linear regression problem where her realized private benefit serves as the response variable and the observed signals for each task act as covariates. However, the observed signals are noisy representations of the agent's true effort, leading to a \textit{measurement error model} \cite{fuller2009measurement}. In classical regression, measurement error in covariates introduces bias, making naive least squares estimators inconsistent and unreliable. This bias arises because the noise in observed signals weakens the correlation between true effort and output, leading to attenuation effects where coefficient estimates are systematically biased toward zero.

To address this issue, we leverage instrumental variable techniques, identifying the contract itself as a valid instrument. Specifically, we propose estimation and learning algorithms based on the \textit{generalized method of moments (GMM)} estimator \cite{alma99653821012205899}. The GMM approach corrects for the endogeneity introduced by measurement error by exploiting moment conditions that remain valid despite the noise. Furthermore, when repeated observations are available, they can serve as additional instrumental variables, enhancing estimation accuracy. The effectiveness of this method is particularly pronounced when agents exhibit sufficient \textit{diversity} in their responses, facilitating a faster convergence rate to the true parameter. Specifically, we show that the principal can achieve a $\widetilde{O}(d)$ regret in utility loss, even adopting a pure exploitation-type algorithm. 



% I propose two approaches based on the generalized method of moments (GMM) estimator. In the first approach, I observe that the contract can act as a valid instrumental variable in the GMM estimator. The principal then faces the exploration-exploitation problem: she must choose the contract so that the GMM estimator is accurate, while at the same time the contract must be close to the optimal contract. 



%Instead, the firm's owner can observe the total revenue generated by the firm under the manager's management. Informally, the higher the effort the manager puts into the tasks, the higher the revenue will be. Possibly, the principal can also observe a noisy signal 

% \begin{enumerate}
% \item Intro
% \item Problem Description
% \item Uniformity Result
% \item Sequential Decision making
% \item The first two estimators
% \item The estimator with diversity
% \item Conclusion
% \end{enumerate}


==> sec/learning.tex <==
\section{A Simple No-regret Algorithm}
This section describes an algorithm that achieves $O(d\sqrt{T})$ regret. The algorithm is based on the idea of explore-then-commit. In the first $d\sqrt{T}$ rounds, the learner queries each orthogonal basis for $\sqrt{T}$ times. These are the exploration rounds. After the exploration rounds, the learner estimates the parameter $\theta$ according to the GMM estimator. The rest of the rounds will be exploitation rounds, where the learner sets $\beta = \hat{\theta}/k$. 

We make the following assumptions on the shape of the cost functions. 
\begin{assumption}
The cost function satisfies the Inada conditions. 
\end{assumption}
\begin{assumption}
The cost function is smooth and strongly convex. 
\end{assumption}
\begin{assumption}
The parameter $\theta$ is bounded between $[c_{\min}, c_{\max}]$. 
\end{assumption}

\begin{algorithm}
\caption{Explore-then-commit type algorithm}
\begin{algorithmic}
\State $T_0 = d\sqrt{T}$
\For {$t = 1, \dots, T_0$}
    \State // Exploration phase
    \State Query $\beta = (0,0,\dots, 1, 0, \dots, 0)$ for $\sqrt{T}$ times. I.e., query each basis for $\sqrt{T}$ times. 
\EndFor
\State Estimate $\hat{\theta} = (Z'X)^{-1} Z'Y$. 
\For {$t = T_0 + 1, \dots, T$}
    \State // Exploitation Phase
    \State $\beta = \hat{\theta} / k$ each round
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{lemma}
At the end of the exploration phase, $\norm{\hat{\theta} - \theta}_2^2 \le O(d/\sqrt{T})$. 
\end{lemma}
\begin{proof}
Denote $W_i$ to be the average agent's best response. Denote $X_i$ to be the average observed signal. Then
\[
X_i = W_i \pm \frac{1}{T^{1/4}}. 
\]

The estimate of $\theta$ then
\begin{align*}
\hat{\theta}_i = \frac{Y_i}{X_i} = \theta_i \pm \frac{1}{T^{1/4}}. 
\end{align*}

Therefore 
\[
\norm{\hat{\theta} - \theta}_2^2 \le O(d/\sqrt{T}). 
\]

% \szcomment{Skip this proof for now, but the high level idea is that each component is queries for $\sqrt{T}$ times and thus is at most $T^{-1/4}$ away from the true value. } 
% Note that each element of the orthonormal basis is queried for $T_0$ times. Denote $w(\beta_i)$ to be the response when $\beta_i$ is posted. Then the average signal should be close to $w$:
% \[
% x_i = w_i \pm \frac{1}{\sqrt{T_0}}. 
% \]
% Then
% \begin{align*}
% \hat{\theta} = \bar{X}^{-1} \bar{Y}. 
% \end{align*}
% Denote 
% \[
% \tilde{\theta} = W^{-1} \bar{Y}
% \]
% which is OLS on the true covariates. Then $\tilde{\theta} - \theta$ error can be bounded by $1 / \sqrt{T_0}$. 

% The error between 
% \begin{align*}
% \norm{\hat{\theta} - \tilde{\theta}} &= |\bar{X}^{-1} - W^{-1}|\bar{Y} \\
% &\le \frac{1}{\sqrt{T_0}}
% \end{align*}

% Therefor $\norm{\hat{\theta - \tilde{\theta}}} \le \frac{1}{\sqrt{T_0}}$. 

% Next, choose $\beta = ???$ in the exploration phase, then each round can be bounded, total regret is $\sqrt{T}$. 
\end{proof}

\begin{theorem}
Total regret $d\sqrt{T}$. 
\end{theorem}
\begin{proof}
Regret in exploration phase $d\sqrt{T}$. Fix a round $t$. The posted contract satisfies:
\[
\norm{\beta - \beta^*}_2^2 \le O(d\sqrt{T}). 
\]


Denote the optimal induced action by $a^*$, and the induced action in this round by $a_t$. Then
\[
\norm{a^* - a_t}_2^2 \le O(d/\sqrt{T}). 
\]

Therefore, for each round in the exploitation phase, the regret can be bounded by
\[
O(d/\sqrt{T}). 
\]

The total regret is then $d\sqrt{T}$. 

(need smoothness and strong convexity). 
\end{proof}

\begin{remark}
By a result in Shamir 2013, this is actually tight. 
\end{remark}



% \section{Learning}
% \begin{algorithm}
% \begin{algorithmic}
% \For {$t = 1,\dots, T$}
%     \State Perform first-stage linear regression and estimate $k_i$
%     \State Perform second-stage linear regression and estimate $\theta$, there is a confidence ellipsoid. 
%     \State Choose $\beta_i = ...$, observe the signal and the outcome. 
% \EndFor
% \end{algorithmic}
% \end{algorithm}


% \section{Learning no noise}
% \begin{algorithm}
% \caption{Algorithm}
% \begin{algorithmic}
% \State $t = 1$
% \For {}
% \While {$t < T$}
%     \State Estimate $\hat{\theta}$ and form a confidence ellipsoid. 
%     \State Compute the axis endpoitns
%     \State Query the $2d$ axis endpoints, i.e., set the contract
%     \[
%     \beta \in \set{S} / k
%     \]
%     for each element in $S$ once
%     \State Update the confidence ellipsoid. 
%     \State $t := t + 2d$
% \EndWhile
% \end{algorithmic}
% \end{algorithm}

% \begin{lemma}[cite{???}]
% The confidence ellipsoid 
% \[
% \norm{\hat{\theta} - \theta}_{V_t} \le \sqrt{d}
% \]
% \end{lemma}

% \begin{lemma}
% Suppose at the beginning of an epoch, the minimum eigenvalue is $\lambda_{\min}$. Then at the end the minimum eigenvalue can be lower bounded by $\lambda_{\min} + ???$. 
% \end{lemma}
% \begin{proof}
% In this proof, let $V_1$ denote the ellipsoid at the beginning of the epoch, and let $V_2$ denote the ellipsoid at the end of the epoch. Then
% \begin{align*}
% V_2 = V_1 + \sum_{x_i \in S} (\hat{\theta} + x_i) (\hat{\theta}+ x_i)^\top + (\hat{\theta} - x_i) (\hat{\theta} - x_i)^\top \\

% \end{align*}
% Take any unit vector $u$. We will need to show $u^\top V_2 u \ge \lambda_{\min} + ???$. 

% Since $x_i$ form a orthogonal basis, we can write $u$ in the form of
% \[
% u = \sum_i \frac{x_i}{\norm{x_i}} y_i. 
% \]
% And that $\norm{y} = 1$. 

% Then 
% \begin{align*}
% u^T [...] u &= \\
% \end{align*}
% \end{proof}

% \begin{lemma}
% At the end of round $t_0 = 2d\cdot \tau$, the minimum eigenvalue $\lambda_{\min}(V_{t_0}) \ge \sqrt{\tau}$. 
% \end{lemma}
% \begin{proof}
% Suppose at the beginning of 
% \end{proof}

% The reward function under $\beta, x$ is
% \[
% \ip{\theta}{x} - \ip{\nabla c(x)}{x} = \ip{\theta}{x} - k c(x) = ( - )
% \]

% \begin{align*}
% \reg = \ip{\theta}{x} - \ip{\beta}{x}
% \end{align*}


==> sec/notes.tex <==
\section{some notes? }
Consider the following optimization problem
\[
\ip{\theta}{x} - 0.5\ip{x}{x}
\]
What is the optimal regret rate for this problem? 

An upper bound is $d\sqrt{T}$ (?). Is this tight? 

Fixes: 1. show simple regret is 1/T, this seems done

2. show regret is 1/sqrt{T}, this also seems done, at least when c satisfies inada conditions. 

3. lower bound on the regret? This has already been shown to be $1/\sqrt{T}$, see Shamir13. Reason: consider quadratic cost with unknown theta. 

4. So it seems that we need to show regret can be $1/\sqrt{T}$ without inada conditions?  

==> sec/proof_robustness.tex <==

\section{Proof of Robustness Result in \Cref{thm:robustness}}

We will show that for any contract $w$, there exists an non-negative affine contract $\phi$ and compatible distributions $\mathcal{F}$ such that
\[
u(\phi; \cF) \ge u(w; \mathcal{F}). 
\]
Since under an affine contract, the agent's expected payment for any action $a$ remains the same for any distribution, we know
\[
u(\phi) = u(\phi; \cF). 
\]
Moreover, by definition
\[
u(w)\le u(w; \mathcal{F}). 
\]
By the above we know that
\[
u(\beta) \ge u(w). 
\]
Then using \Cref{lem:best-linear}, which shows we can further improve an affine contract to a linear contract, the theorem is proven. 


We define the following set of points:
\[
S = \set{(x, w(x)): x\in \mathcal{X}}. 
\]



For each upper hyperplane $H$ supporting the set $S$ from above, consider the set of points that the plane $H$ supports, and project these points back to the space $\mathcal{X}$. Denote this set as $P(H)$. By definition $P(H)\subset \mathcal{X}$. 

% \begin{lemma}

% There exists a  

% \end{lemma}



% define $C(H)$ as the set of points in $S$ that . Define $C(H)$ as the projection of $S(H)$ onto the signal space and taking the convex hull(?). Let $\mathcal{H}$ to be the set of all upper supporting hyperplanes, which we can assume to be compact and convex. 



% \begin{lemma}

% There exists a family of hyperplanes which touch the set $S$ from above, and that $\cup_{H \in \mathcal{H}} \conv(P(H)) = \conv( \mathcal{X} )$. 

% \end{lemma}

% \begin{proof}



% \end{proof}


By a classic result in convex geometry (e.g. \cite{lee2017subdivisions}, \cite{de2010triangulations}), if we consider the set of upper facets of the set $S$ (for which each defines an upper hyperplane), projecting each facet back to $\mathcal{X}$ in fact gives an exact partition of $\mathcal{X}$, i.e., 
\[
\cup_{H: H \text{ touches an upper facet}} \conv(P(H)) = \conv(\mathcal{X}). 
\]

For our purposes, we will be considering upper supporting hyperplanes whose normal vector's last component is bounded away from 0. lower bounded by some $\eps$. In the following denote $n_{d+1}(H)$ to as the last component of the normal vector. For hyperplanes with $n_{d+1}(H) = 0$, they do not represent valid contracts. 

% It can be seen that if we take the set of all hyperplanes which bound $H$ from above, and project each such hyperplane to the 'unlifted' signal space $\mathcal{X}$, then the union of the projections recovers the set $\mathcal{X}$. For our purposes, we impose a lower bound on the last component of the normal vector of hyperplanes which bound $S$ from above. We summarize this into the below lemma. 

% Alternatively, for each point $x_0$, there exists a hyperplane $H$ whose support after dropping the last 'height' component $w()$ is $x_0$. 



\begin{lemma}
\label{lemma:triangulation}
There exists some $\eps>0$, such that if we define $\mathcal{H} = \set{H: n_{d+1}(H)\ge \eps}$, then
\[
\cup_{H \in \mathcal{H}} \conv(P(H)) = \conv( \mathcal{X} ). 
\]
\end{lemma}
\begin{proof}
The set $S$ has at most a finite number of upper facets, to which each corresponds to a hyperplane $H$. Then, simply set $\eps$ to be the minimum of $n_{d+1}(H)$ among all such $H$, and the lemma is proven. 
\end{proof}

Now, it can be seen that the set $\mathcal{H}$ as in the previous lemma is topologically equivalent to a closed and convex set. This will allow us to apply fixed-point theorems in the subsequent analysis. 

In the following, we define $\phi(H)$ to be the affine contract associated with the hyperplane $H$, and use $a(H) = a(\phi(H))$ to denote the action that is induced by $\phi(H)$. 
\begin{lemma}
There exists an upper supporting hyperplane $H$, such that the incentivized action $a^*$ under $\phi(H)$ lies in the set $\conv(P(H))$. 
\end{lemma}
Recall this is the notion of ``self-owned" hyperplanes as introduced previously. 

\begin{proof}
By the previous lemma, the union of all $\conv(P(H))$ cover the entire space $\mathcal{A}$. Then for any $a$, there must exist some hyperplane $H'$, such that $a(H)\in \conv(P(H'))$. 

So, let us define a function $g:\mathcal{H}\rightarrow 2^\mathcal{H}$, such that for each upper supporting hyperplane $H$, the function maps to a set of supporting hyperplanes defined as follows:
\[
g(H) = \set{H': a(H) \in \conv(P(H'))}
\]
By the previous lemma, the set $g(H)$ is non-empty. Further, we can see that the set $g(H)$ is convex and that $g$ has a closed graph (see \Cref{app:Kakutani} for a brief discussion). By Katukani's fixed point theorem, there exists some hyperplane $H$ such that $g(H) = H$. Hence the theorem is proven. 
% Note that the agent's best response $a(H)$ is continuous with respect to $H$ (or more precisely with respect to $\beta(H)$).  Then, there must exists such a mapping $g$ which is continuous. 
\end{proof}

We can now show that there exists some affine contract which does no worse than $w$ in worse-case. 
\begin{lemma}
Let $H$ be the hyperplane as in the statement of the previous lemma (i.e., ``self-owned") and $H$ induces $a(H)$. Then there exists some distribution under which the contract $w$ also induces $a(H)$. Further, $\phi(H)$ uses no greater payment than $w(\cdot)$. 
\end{lemma}

\begin{proof}
First note that under any distribution, for any action $a\in \mathcal{A}$, the payment to the agent under $w$ is certainly no larger than under $\phi$, since $\phi$ bounds $w$ from above. Now, since $H$ is ``self-owned", we have $a(H) \in \conv(P(H))$. We can define a compatible distribution where the signal distribution of action $a(H)$ is supported only on points in $P(H)$. For points $x\in P(H)$ we have $\phi(x) = w(x)$. Then, the payment to the agent if he takes action $a(H)$ is exactly the same under $\phi(H)$ as under $w(\cdot)$. Hence, under this distribution, the contract $w$ also induces action $a(\beta)$. 
\end{proof}

Thus so far, we have shown that any contract $w(\cdot)$ can be improved to an affine contract whose worst-case payoff is no less than that of $w(\cdot)$. By \Cref{lem:best-linear}, any affine contract can be improved to a linear contract. This completes the proof. 

% Without loss of generality we can assume the induced action is not the $0$ vector; otherwise the principal can simply use the $0$ contract. 

% \begin{lemma}
% If the affine contract $\phi$ induces action $a^* = a(\beta')$ and $a\neq 0$, then the linear contract $\beta = \nabla c(a)$ induces $a$ at a no greater cost. 
% \end{lemma}
% \begin{proof}
% Given any affine contract $\beta'$, the agent's maximization problem is:
% \[
% \max_{a} \sum_i \phi_i a_i - c(a). 
% \]
% Clearly, the above is a concave function of $a$. Since $a^*$ is the maximizer to the above, by first-order optimality condition, we know that the below must hold. 
% \[
% \ip{\phi - \nabla(a^*)}{a - a^*} \le 0, \forall a\in\mathcal{A}. 
% \]
% Now, let us take $a = a^* / 2$. Then by the above, we directly get
% \[
% \ip{\phi - \nabla(a^*)}{ -0.5 a^*} \le 0, 
% \]
% which directly implies 
% \[
% \ip{\phi }{a^*} \ge \ip{\nabla c(a^*)}{a^*}. 
% \]
% Hence $\nabla c(a^*)$ induces effort profile $a^*$ at a strictly lower cost. 
% \end{proof}

Our main result in this section $\Cref{thm:robustness}$ then follows from the above lemmas. 

\begin{remark}
Our results can also be extended to the case when the signal space is infinite, e.g., $\mathcal{X} = [0,1]^d$. However, this requires some additional regularity assumptions. In particular, we need to ensure the contract does not grow ``too quickly" at the boundary. This avoids the case that at the boundary a ``vertical" supporting hyperplane occurs, i.e., one with $n_{d+1}(H) = 0$. Such hyperplanes does not correspond to valid contracts, and \Cref{lemma:triangulation} does not hold. 
\end{remark}



% \szcomment{DON'T use below. }

% \begin{lemma}
% There exists some $S_i$, such that the incentivized action $a^*$ under the contract $\beta(w; S_j)$ belongs to the convex hull of $S_i$. 
% \end{lemma}



% \begin{proof}

% For sake of contradiction suppose not, that is for each triangulation induced new affine contract, the induced action is in some other triangulation. Suppose there is a total of $M$ triangulations. Then there must exists a sequence of triangulations, such that the triangulation in id $i$ falls in id $i+1$. 



% Then, let each incentivized action be only supported by the vertices on the triangulation. We have the following

% \[
% \sum_{j} p_{i+1,j} w'_{i+1,j} - c(a_{i+1}) \ge \sum_{j} p_{i,j} w_{i,j} - c(a_i)
% \]

% % We sum over all such inequalities

% % \[

% % \sum_{j} p_{i+1,j} w'_{i+1,j} - c(i+1) \ge \sum_{j} p_{i,j} w_{i,j} - c(i)

% % \]

% Sum over all, then

% \[
% \sum_i \sum_{j} p_{i+1,j} w'_{i+1,j} > \sum_i \sum_{j} p_{i,j} w_{i,j}
% \]

% But we know that $w'_{i+1, j} \le w_{i,j}$, and that at least one term is strict:

% \[
% \exists i, j, p_{i, j} w'_{i+1, j} < p_{i,j} w_{i,j}. 
% \]

% Hence we obtain a contradiction, and the lemma is proven. 

% \end{proof}

% \begin{remark}
% Our methods can also extend to the case to when there are infinite number of outcomes. 
% \end{remark}

==> sec/robustness.tex <==
\section{Robustness in Ambiguous settings}

Here, we explore the robustness properties of linear contracts in an ambiguous setting. In particular, we show that linear contracts are worst-case optimal in environments where only the mean outcomes of each action are known.

In this section, we assume that tasks generate binary signals, with the signal space denoted as $\mathcal{X} = \set{0,1}^d$. The agent's action space is given by $\mathcal{A} = [0,1]^d$. When the agent takes an action $a \in \mathcal{A}$, the expected signal for task $i$ is $a_i$, and the agent incurs a cost $c(a)$. 

The principal seeks to guarantee a worst-case payoff in an ambiguous setting where the exact distribution of each action is unknown. To formally define the worst-case payoff, we first introduce the concept of \emph{compatible distributions}.


\begin{definition}

We say a family of distributions $\mathcal{F} = \set{ a \in \mathcal{A} | F_a \in \Delta(\bbR^d) } $ is compatible if for each $a\in \mathcal{A}$, we have

\[
\Ex_{x\sim F_a}[x]. 
\]

\end{definition}

A contract by a principal is a mapping from all possible outcomes to a payment, which we denote by $w: \mathcal{X} \rightarrow \bbR^+$. Note that the agent is protect by limited liability. The worst-case payoff for the principal in an ambiguous setting is defined as
\begin{align}
u(w) = \min_{\mathcal{F} \text{ is compatible}} u(w; \mathcal{F}) \label{eq:robustnessObj}
\end{align}

Here $u(w;\cF)$ is the principal's payoff using contract $w$ assuming the agent's true distributions were $\cF$ and that the agent best responds to the contract $w$. 


We show that there is a linear contract $\beta\in \mathbb{R}^d$ maximizing the above expression. Recall that under the linear contract $\beta$, the agent's payment under signal $x$ is

\[
\beta(x) = \sum_{i=1}^d \beta_i x_i. 
\]

\begin{theorem}
\label{thm:robustness}
There exists a linear contract maximizing the principal's worst-case objective as given in $\cref{eq:robustnessObj}$. 
\end{theorem}

\begin{remark}
    Although we assume tasks have binary signals in $\set{0,1}$, our results extend to more general settings where the signal for each task can take any finite number of values. Furthermore, under mild regularity conditions, these results also apply when the signal space is continuous. 
\end{remark}

% The model we will be working with will be different from the previous sections which provided the uniformity result and ... Actions are distribution-ambiguous, meaning that $a\in\mathcal{A}$, the expected outcome 





%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%



% \subsection{Ambiguous in distribution for $d = 2$}

% Here we show robustness results in an ambiguous principal-agent setting. 



% We consider a setting where there are 2 tasks, and that either task can succeed or fail, so that there is a total of 4 outcomes. 



% We show that under an ambiguous principal-agent setting, the optimal contract must be of the form

% \[

% w(y) = \beta_0 + \beta_1 \ind{y_1 = 1} + \beta_2 \ind{y_2 = 1}. 

% \]



% \begin{theorem}

% Given an ambiguous principal agent setting with a set of actions $A$. Given any contract $w(\cdot)$, there exists a contract $\beta$ in the family of affine contracts, such that there exists a family of compatible distribution (recall distribution is for each action), such that the payoff of $\beta$ to the principal is no less than that of $w(\cdot)$. 

% \end{theorem}



% \begin{proof}

% There are two cases. First case is that $s(1,1) > s(0,0) + s(0,1) - s(0,0)$. 



% Second case is that $s(1,1) < s(1,0) + s(0,1) - s(0,0)$. 



% In the first case, we lower either the payoff for $s(1,1)$ or $s(0,0)$. And show that at least in one of the two affine contracts, the optimal action $a^*$'s payment in the 2 schemes will remain the same. This is because, at least in one of the two schemes, the action $a^*$ will be in the convex hull whose payoff did not change. 



% In the 2nd case, we lower either the payoff for $s(1,0)$ or $s(0,1)$. And show that at least in one of the two newly formed affine contracts, the optimal action $a^*$'s payment in the 2 schemes will remain the same. 

% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof Sketch}
Let's first focus on affine contracts. We show that there exists an affine contract that maximizes the principal’s worst-case objective. A key property of affine contracts is that under any family of compatible distributions over outcomes, the agent’s best response remains unchanged---so the principal’s payoff is independent of the particular distribution in that family. Then in the last step, we improve the affine contract to a linear contract. 

Our strategy consists of the following steps. 

\medskip

\paragraph{\bf From a Non-affine Contract to an Affine Contract.} 

Given any (possibly non-affine) contract \(w(\cdot)\), we will construct an affine contract \(\phi\) and identify a corresponding family of compatible distributions \(\mathcal{F}\) such that the principal’s payoff under \(\phi\) is at least as high as under \(w\) for the compatible distribution family \(\mathcal{F}\). Since the payoff from an affine contract does not depend on the particular choice of distribution family \(\mathcal{F}\), it follows that the worst-case objective achieved by some affine contract is at least as good as that achieved by \(w(\cdot)\).

\medskip

\paragraph{\bf A Family of Affine Contract via Upper Supporting Hyperplanes.} To obtain the affine contract, we upper-bound \(w(\cdot)\) by finding an affine function \(\phi\) that satisfies
\[
\phi(x) \ge w(x) \quad \text{for all } x.
\]
Consider the \emph{lifted set}
\[
S = \{ (x, w(x)) : x \in \mathcal{X} \}.
\]
For any hyperplane \(H\) that supports \(S\) from above (an \emph{upper supporting hyperplane}), we can associate an affine contract \(\phi(H)\) that satisfies the inequality above. In this way, \(\phi(H)\) serves as an upper bound to the payment function \(w\).

\medskip

\paragraph{\bf ``Self-Owned" Hyperplanes.} 
We now introduce the notion of a \emph{self-owned hyperplane}: a hyperplane \(H\) is called \emph{self-owned} if the induced action \(a(H)\) under the affine contract \(\phi(H)\) lies in the convex hull of its own contact set (after projected back to $\mathcal{X}$), that is,
\[
a(H) \in \operatorname{conv}(P(H)).
\]
Here we define
\[
P(H) = \{ x \in \mathcal{X} : (x, w(x)) \in H \}. 
\]
When \(H\) is self-owned, one may choose a compatible distribution where the support of taking action $a(H)$ is only supported on \(P(H)\). Then, since $H$ touches the $S$, we know that the agent’s payment is identical under both \(w\) and \(\phi(H)\). This means that if the affine contract $\phi(H)$ induced action $a$, then under this compatible distribution the non-affine contract $w(\cdot)$ also induces action $a$, and that $\phi(H)$ induces $a$ at a no larger payment. 

% For the affine contract \(\phi(H)\) to be effective, we need that for the action \(a\) chosen by the agent, the payment under \(\phi(H)\) coincides with that under \(w\), i.e.,
% \[
% \phi(H)(a) = w(a).
% \]
% This equality can be ensured if the distribution of outcomes when the agent takes action \(a\) lies entirely on the set of points where \(H\) touches \(S\). Define
% \[
% P(H) = \{ x \in \mathcal{X} : (x, w(x)) \in H \},
% \]
% as the projection of these contact points onto \(\mathcal{X}\).


\medskip

\paragraph{\bf Existence of a Self-Owned Hyperplane. } A classical result in convex geometry (e.g. \cite{lee2017subdivisions}) implies that the union of the convex hulls of \(P(H)\) over all upper supporting hyperplanes \(H\) covers the entire outcome space \(\mathcal{X}\). In particular, for every action \(a \in \mathcal{X}\) there exists some hyperplane \(H\) such that \(a \in \operatorname{conv}(P(H))\). Then, we can construct a set-valued mapping:
\[
g: \mathcal{H} \to 2^\mathcal{H},
\]
defined as
\[
g(H) = \set{H': a(H) \in \conv(P(H'))}. 
\]
By applying Kakutani's fixed point theorem (\cite{kakutani1941generalization}), there exists a hyperplane \(H^*\) such that
\[
H^* \in g(H^*).
\]
Then we have precisely found a self-owned hyperplane. 

%This fixed point \(H^*\) is self-owned, meaning that the action incentivized by \(\phi(H^*)\) is supported on \(P(H^*)\). Consequently, by choosing a compatible distribution supported on \(P(H^*)\), the agent receives the same payment under both \(w\) and \(\phi(H^*)\).

\medskip

\paragraph{\bf Refining to a Linear Contract.} Finally, we show that if the affine contract \(\phi\) induces an action \(a^*\), then there exists a linear contract (i.e., one with zero offset) that also induces \(a^*\) while providing no greater payment to the agent. This completes the proof by establishing that within the class of contracts, a linear contract exists that maximizes the principal’s worst-case objective. 

\medskip

By these steps, we conclude that for any arbitrary contract \(w\), there is a linear contract that performs at least as well in the principal’s worst-case evaluation. This completes the proof sketch. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Remove my own proof idea
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Proof Idea}
% In this section, we briefly outline the idea behind the theorem. 

% We first show that there exists an affine contract maximizing the principal's worst-case objective. An affine contract is a linear contract with the addition of an ``offset" parameter. We use $\phi\in \bbR^{d+1}$ to represent an affine contract, and under this contract, the agent's payment function is $\phi(x) = \phi_0 + \sum_{i=1}^d \phi_i x_i$. First note that under an affine contract, the agent's best response will be the same for any compatible distribution, and hence yielding the principal the same payoff for any compatible distribution. 

% Now, given a non-affine contract $w(\cdot)$, we shall find an affine contract $\phi$ and a compatible distribution family $\cF$, such that the payoff of $\phi$ to the principal is no less than the payoff of $w(\cdot)$ under the compatible distribution family $\cF$. Then, since affine contracts yields the same payoff for any compatible distributions, this means $u(\beta) \ge u(w)$. Finally, given an affine contract $\phi$, we show that there must exists a linear contract $\beta$ which strictly improves upon the affine contract. Showing these completes the proof. 

% To proceed, we will find an affine contract $\phi$ whose payments are no less than those of $w$ for each possible outcome, in other words, $\phi$ is going to bound the function $w$ from above. To do so, we find all upper supporting hyperplanes for the lifted space $S = \set{ (x, w(x)) }$. Each of the upper supporting hyperplanes $H$ corresponds to a possible affine contract $\phi(H)$ which bounds $w$ from above. Now, for any action $a$ that the agent can take, he receives a no greater payment under $w$ than under $\phi(H)$. 

% So how to show existence of this hyperplane $H$? If we want the action $a(H)$ to have the same payment under $\alpha(H)$ and under $w$, then it suffices for the distribution of action $a(H)$ to only lie on the support of the hyperplane $H$ that touches the set $S = (x, w(x))$. In other words, it suffices for $a(H)$ to lie inside the convex hull of the support of $H$ (after projecting back to the ``unlifted set" $\mathcal{X}$. )

% Our next goal is to show that there exists some hyperplane $H$, with associated affine contract $\phi(H)$, and some specific compatible distributions $\cF$, such that for the incentivized action $a$ under $\phi(H)$, taking action $a$ gives the agent the same payment under $\phi(H)$ and under $w$. Hence, $\phi(H)$ and $w$ must incentivize the same action $a$ under this specific distribution $\cF$. From this, we know that the affine contract $\alpha(H)$ does no less than $w$ in the worst case. 



% Let us elaborate on the existence of such an affine contract and compatible distribution. For each possible upper supporting hyperplane $H$, let us consider the set of points on the support of $H$ and project these points back to $\mathcal{X}$, call this set $P(H)$. By a classic result in convex geometry, the union of the convex hulls of $P(H)$ over all $H$ is exactly the possible signal space $\mathcal{X}$. In other words, for each point $a\in \mathcal{A}$, there exists some hyperplane $H$ such that $a$ belongs to the convex hull of $P(H)$. Consider the function $g:\mathcal{H}\rightarrow \mathcal{H}$ which map a hyperplane $H$ to another hyperplane $H'$, such that the induced action $a$ under the affine contract associated with $H$ must belong to the convex hull of $P(H')$. Then, by a fixed-point theorem, there must exist some hyperplane $H$, such that the incentivized action under the affine contract associated with $H$ must lie within the convex hull of itself, $P(H)$. This precisely shows that we can let the compatible distribution be such that the action $a$ is only supported on the points in $P(H)$, and hence the payment for taking action $a$ remains the same under the affine contract and under $w$. 



% As the last step, we should that if the affine contract induces some action $a^*$, then there must exist a linear contract induces $a^*$ with a no greater payment to the agent. This finishes the proof. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%   END
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\textwidth]{media/plot_robust_new.png}
%     \caption{Illustration of the lifted set. The lifted set loosely resembles a square being foled slightly along the diagonal}
%     \label{fig:vis_robust}
% \end{figure}


\subsection{An Example}
We illustrate the key ideas, in particular, the existence of a self-owned hyperplane, with a concrete example. 

Consider a setting with \(d=2\) and the following non-affine (non-linear) contract \(w\) defined on \(\mathcal{X} = \{0,1\}^2\):
\[
w(0,0)=0,\quad w(1,0)=2,\quad w(0,1)=2,\quad w(1,1)=3.
\]
We \emph{lift} the space \(\mathcal{X}\) into \(\mathbb{R}^3\) by appending the contract value as a third coordinate. In other words, we consider the set
\[
S = \{(0,0,0),\ (1,0,2),\ (0,1,2),\ (1,1,3)\}.
\]
If \(w\) were affine, then \(S\) would lie on a single hyperplane in \(\mathbb{R}^3\). Since \(w\) is not affine, \(S\) forms a polytope with several facets. In particular, there are two \emph{upper facets} of \(S\) that yield upper supporting hyperplanes, each corresponding to an affine contract that upper bounds \(w\).

One such upper facet defines an affine contract \(\phi_1\) with
\[
\phi_1(0,0)=0,\quad \phi_1(1,0)=2,\quad \phi_1(0,1)=2,\quad \phi_1(1,1)=4.
\]
This hyperplane touches \(S\) at the points
\[
X_1 = \{(0,0),\ (1,0),\ (0,1)\}.
\]
Similarly, another upper facet defines an affine contract \(\phi_2\) given by
\[
\phi_2(0,0)=1,\quad \phi_2(1,0)=2,\quad \phi_2(0,1)=2,\quad \phi_2(1,1)=3,
\]
supported on the points
\[
X_2 = \{(1,0),\ (0,1),\ (1,1)\}.
\]
Note the triangulation is clearly illustrated: $\mathcal{X} = \conv(X_1)\cup \conv(X_2)$. 

Besides the two upper facets, any convex interpolation between these two hyperplanes also yields a valid supporting hyperplane for \(S\). Such interpolated hyperplanes are supported on the two endpoints \((1,0)\) and \((0,1)\).

We now claim that there must exist at least one hyperplane among these—one that we call \emph{self-owned}—for which the induced action lies within its own set of support points (after projecting back to \(\mathcal{X}\)). In other words, if \(H\) is the hyperplane corresponding to an affine contract \(\phi(H)\), define
\[
P(H)=\{x\in \mathcal{X} \mid (x,w(x))\in H\}.
\]
Then \(H\) is \emph{self-owned} if the action \(a\) induced by \(\phi(H)\) satisfies
\[
a \in \operatorname{conv}(P(H)).
\]

Suppose, for the sake of contradiction, that no self-owned hyperplane exists. Then the affine contract \(\phi_1\) would induce an action falling in \(X_2\) while \(\phi_2\) would induce an action in \(X_1\). However, the mapping from the hyperplane to the induced action is continuous (small changes in the hyperplane lead to small changes in the induced action). Therefore, as one continuously interpolates between \(\phi_1\) and \(\phi_2\), the induced action must eventually lie exactly in the convex combination (or “interval”) determined by \((1,0)\) and \((0,1)\). Note that here Kakutani's fixed point theorem reduces to an intermediate value theorem. Hence, this guarantees the existence of a self-owned hyperplane.

% Once such a self-owned hyperplane \(H\) is identified, one can construct a compatible distribution whose support is contained in
% \[
% P(H)=\{x\in \mathcal{X} \mid (x,w(x))\in H\}.
% \]

% On these points, the affine contract \(\phi(H)\) and the original contract \(w\) yield the same payments. Moreover, since \(\phi(H)\) upper bounds \(w\) over all outcomes, any deviation yields no higher payment. Therefore, for this compatible distribution, the affine contract induces the same action as \(w\) with no greater payment, demonstrating that the affine contract performs at least as well as the original non-affine contract.

% This example captures the essence of our general proof: starting from any non-affine contract, one can employ the geometry of the lifted space and the notion of self-owned hyperplanes to construct an affine (and, ultimately, a linear) contract that is optimal for the principal’s worst-case objective. 



%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Remove my old example
%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{An Example OLD}
% Before giving the proof to the theorem, we walkthrough a concrete example illustrating the proof idea. We start with a specific non-affine contract and show how to turn it into an affine contract, such that the affine contract performs no worse than the non-affine contract for some distribution. 

% Consider a setting with $d=2$ with a non-affine and non-linear contract $w$ as specified below. 
% \[
% w(0,0) = 0, w(1,0) = 2, w(0,1) = 2, w(1,1) = 3. 
% \]
% We can ``lift" the space $\mathcal{X} = \set{0,1}^2$ into $\bbR^3$ by appending the value of $w(x)$ as the last coordinate. In other words, the lifted space is the polytope defined by
% \[
% S = \set{ (0,0,0), (1,0,2), (0,1,2), (1,1,3) }. 
% \]
% If the contract were affine, the lifted polytope would just be a hyperplane. But of course the contract $w$ is not affine. There are two upper facets of $S$, each of which defines a hyperplane that bounds $S$ from above, the corresponding affine contracts are
% \[
% w(0,0) = 0, w(1,0) = 2, w(0,1) = 2, w(1,1) = 4,
% \]
% which is supported on the three points $X_1 = \{(0,0), (1,0), (0,1) \}$ in $\cX$. 
% and
% \[
% w(0,0) = 1, w(1,0) = 2, w(0,1) = 2, w(1,1) = 3, 
% \]
% which is supported on the three points $X_2 = \{(1,0), (0,1), (1,1) \}$ in $\cX$. 
% The interpolation between the two hyperplanes are also valid hyperplanes; these hyperplanes are supported on the two endpoints $(1,0)$ and $(0,1)$. 

% We claim that there must exist some hyperplane such that the induced action belongs to it's own support points after being projected back to $\cX$; call such a hyperplane ``self-owned". Suppose not, then the affine contract $w_1$ induces some action in $X_2$, and the affine contract $w_2$ induces some action in $X_1$. At the same time, the induced action is continuous in the sense that if we perturb the affine contract slightly, the induced action should not change much. Hence, as we continuously interpolate between $w_1$ and $w_2$, somewhere the induced action must fall exactly into the interval defined by $(1,0)$ and $(0,1)$, and hence we always have a ``self-owned" hyperplane. 

% Once we have such a ``self-owned" hyperplane $H$, we can construct compatible distributions where the support of the action $a$ is supported only on the support of $H$. On these points, the payment of the affine contract shares exactly the same payments as the original non-affine contract $w$. Further, since the affine contract bounds $w$ from above, any action receives a no greater payment. As such the affine contract induces the same action with no greater payment, and is no worse off then $w$ for this distribution. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% END Example OLD
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Then, by applying a fixed-point theorem, we can show that there must exists a hyperplane $H$ under which the incentivized action under the affine contract lies inside the support of the hyperplane $H$. Then, we can corresponding construct a distribution associated with the incentives action $a^*$, such that $a$ is only supported on the support of $H$, hence the payment for taking action $a^*$ remains the same under $w$ and under the affine contract defined by the hyperplane $H$. Further, since $H$ bounds $w$ from above, any action receives a no greater payment. Hence, action $a^*$ is incentives under the affine contract and at the same payment. 



% We will argue that for a carefully chosen distribution family, the incentivized action under $\beta$ is the same as the incentized action under contract $w()$. Note that for each action $a$, the agent receives a no greater payment under $w$ than under $\beta$. Moreover, we can carefully construct some distribution so that the payment of action $a^*$ is the same under the two contracts. suppose that the incentived action under $\beta$ is $a^*$, then we construct a compatible distribution $\cF$ and make it so that in the compatible distribution, the action $a^*$ is only supported on unchanged outcomes, i.e., for outcomes $x$ which $\beta(x) = w(x)$. Hence, the payment of $a^*$ remain unchanged. Then, the affine contract also incentivizes $a^*$ with the same payment, and must perform no worse than the contract $w(\cdot)$. 

% We now describe how one can construct such an affine contract. Recall the set of outcomes is $\mathcal{X} = [0,1]^d$, and that $w(\cdot)$ is a mapping from each possible outcome to a payment. We perform the so-called lifting operation and obtain a set of points in the $\bbR^{d+1}$ space:

% \[
% \set{ x\in\mathcal{X} : (x, w(x)) }. 
% \]

% Considering the set of facets on the lower convex hull of the set of points, if we project the facet back to the outcome space, they form a partition of the outcome space $\mathcal{X}$. Let the partition be $\set{ S_1, \dots, S_m }$, where each $S_i$ is a set of points in the original outcome space $\set{0,1}^d$, so that $\cup conv(S_j) = [0,1]^d$. 



% Now suppose we have obtained this partition (or triangulation). Each set $S_j$ corresponds to a lower facet in the lifted space, and represents a possible way to modify the contract: we can define the affine contract as being the hyperplane defined by this facet. Note that given a triangulation, only vertices that are outside the triangulation have their values decreased. The final step is then to show that there exists a lower facet, such that the incentivized action, call it $a^*$, under the modified contract as defined by $S_j$ must belong to the convex hull of $S_j$. Then, we can construct a compatible distribution such that $a^*$ is only supported on the points in $S_j$, and hence the payment to the agent if he should take $a^*$ remains unchanged. Therefore, recall that since $\beta < w$, the payment for any action does not increase and the payment for action $a^*$ is the same, $a^*$ is still incentivized under the affine contract. Hence the principal's under the affine contract $\beta$ must be no less than that under $w$. 





